Information geometry of excess and housekeeping entropy production

A nonequilibrium system is characterized by a set of thermodynamic forces and fluxes which give rise to entropy production (EP). We show that these forces and fluxes have an information-geometric structure, which allows us to decompose EP into contributions from different types of forces in general (linear and nonlinear) discrete systems. We focus on the excess and housekeeping decomposition, which separates contributions from conservative and nonconservative forces. Unlike the Hatano-Sasa decomposition, our housekeeping/excess terms are always well-defined, including in systems with odd variables and nonlinear systems without steady states. Our decomposition leads to far-from-equilibrium thermodynamic uncertainty relations and speed limits. As an illustration, we derive a thermodynamic bound on the time necessary for one cycle in a chemical oscillator.

==> preamble.tex <==
\setcounter{secnumdepth}{3}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{newtxtext}
\usepackage{stmaryrd}
\usepackage{titlesec}
\usepackage{float}

\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.
\DeclareMathOperator*{\argmin}{\arg\,\min}
\DeclareMathOperator*{\argmax}{\arg\,\max}

%\let\oldbibliography\bibliography 
% \renewcommand{\bibliography}[1]{
% \renewcommand{\ref}{\oldref}
% \oldbibliography{#1}
% \renewcommand{\ref}{\cref}
% }


% \usepackage[capitalize]{cleveref}
% \AtBeginDocument{
% \let\oldref\ref
% \renewcommand{\ref}{\cref}
% }

% \crefname{thm}{Theorem}{Theorems}
% \crefname{lem}{Lemma}{Lemmas}
% \crefname{prop}{Proposition}{Propositions}
% \crefname{defn}{Definition}{Definitions}
% \crefname{rem}{Remark}{Remarks}

\usepackage{color}% for colors
\RequirePackage[dvipsnames,usenames]{xcolor}

\pdfstringdefDisableCommands{%
  \renewcommand{\bm}[1]{#1}%
}

\makeatother
\allowdisplaybreaks


\global\long\def\bath{\alpha}%
\global\long\def\epr{\dot{\sigma}}%
\global\long\def\eprHK{\epr_{\text{hk}}}%
\global\long\def\eprEX{\epr_{\text{ex}}}%
\global\long\def\eprhsHK{\epr_{\text{hk}}^{\text{HS}}}%
% 
\global\long\def\eprhsEX{\epr_{\text{ex}}^{\text{HS}}}%
\global\long\def\ee{\bm{\theta}}%
\global\long\def\cc{\bm{c}}%
\global\long\def\ff{\bm{f}}%
% 
\global\long\def\zz{\bm{0}}%
% 
\global\long\def\rr{\rho}%
% 
\global\long\def\dt{\mathrm{d}_{t}}%
\global\long\def\BBdiv{\nabla^{T}}%
\global\long\def\BBgrad{\nabla}%
\global\long\def\negBBgrad{{-\nabla}}%
\global\long\def\TJ{J}%
\global\long\def\jj{\bm{\TJ}}%
\global\long\def\jjrr{\TJ_{\rr}}%
% 
\global\long\def\negedge{\tilde \rr}
%\global\long\def\jjRev{\tilde{\bm{\TJ}}}%
%\global\long\def\jjjrr{\tilde{\TJ}_{\rr}}%
\global\long\def\jjEdgeNegRev{\TJ_{\negedge}}%
%\global\long\def\jjjEdgeNegRev{\tilde{\TJ}_{\negedge}}%
\global\long\def\PJ{j}%
\global\long\def\jjT#1{\bm{\PJ}(#1)}%
\global\long\def\jjrrT#1{\PJ_{\rr}(#1)}%
\global\long\def\pot{\bm{\phi}}%
\global\long\def\eerr{\theta_{\rr}}%
% 
\global\long\def\ffrr{f_{\rr}}%
\global\long\def\DD{\mathcal{D}}%
\global\long\def\dKL{D_{\mathrm{KL}}}%
% 
\global\long\def\numstate{N}%
% 
\global\long\def\numedge{M}%
% 
\global\long\def\ep{\Sigma}%
\global\long\def\epEX{\ep_{\mathrm{ex}}}%
\global\long\def\epHK{\ep_{\mathrm{hk}}}%
\global\long\def\pp{\bm{p}}%
\global\long\def\dtp{\dt\pp}%
\global\long\def\qq{\bm{q}}%
% 
\global\long\def\LLL{\mathcal{L}}%
\global\long\def\taumin{\tau_{\mathrm{min}} }%
\global\long\def\eerrR{\theta_{\negedge}}%
\global\long\def\ffrrR{f_{\negedge}}%
\global\long\def\netflux{\bm{\mathcal{J}}}%
\global\long\def\obs{\pot}%
% 
\global\long\def\chngObs{\mathcal{J}_{\bm{\phi}}}%
% 
\global\long\def\FFF{\Phi}%
% 
\global\long\def\actOBS{\mathcal{V}_{\obs}}%
\global\long\def\oddconj{\epsilon}%
\global\long\def\timedepJ{\mathcal{J}_{\obs}^{t}}%
\global\long\def\timedepA{\mathcal{V}_{\obs}^{t}}%
\global\long\def\atanh{\tanh^{-1}}%



\usepackage{babel}

